Exact Byzantine Consensus on Undirected Graphs under Local Broadcast Model

This paper considers the Byzantine consensus problem for nodes with binary inputs. The nodes are interconnected by a network represented as an undirected graph, and the system is assumed to be synchronous. Under the classical point-to-point communication model, it is well-known [7] that the following two conditions are both necessary and sufficient to achieve Byzantine consensus among $n$ nodes in the presence of up to $f$ Byzantine faulty nodes: $n \ge 3f+1$ and vertex connectivity at least $2f+1$. In the classical point-to-point communication model, it is possible for a faulty node to equivocate, i.e., transmit conflicting information to different neighbors. Such equivocation is possible because messages sent by a node to one of its neighbors are not overheard by other neighbors. This paper considers the local broadcast model. In contrast to the point-to-point communication model, in the local broadcast model, messages sent by a node are received identically by all of its neighbors. Thus, under the local broadcast model, attempts by a node to send conflicting information can be detected by its neighbors. Under this model, we show that the following two conditions are both necessary and sufficient for Byzantine consensus: vertex connectivity at least $\lfloor 3f/2 \rfloor + 1$ and minimum node degree at least $2f$. Observe that the local broadcast model results in a lower requirement for connectivity and the number of nodes $n$, as compared to the point-to-point communication model. We extend the above results to a hybrid model that allows some of the Byzantine faulty nodes to equivocate. The hybrid model bridges the gap between the point-to-point and local broadcast models, and helps to precisely characterize the trade-off between equivocation and network requirements.

==> hybridFaultsAlgo.tex <==
%!TEX root = ConsensusBroadcastUndirected.tex


As in proof of Theorem \ref{theorem necessity}, the necessity proof is tackled in two parts corresponding to the two network conditions (condition (ii) is implied by Theorem \ref{theorem necessity}).
For sufficiency, we modify Algorithm \ref{algorithm consensus} for the hybrid setting.
The formal procedure is given in Algorithm \ref{algorithm hybrid consensus}.
A proof of correctness appears in Appendix \ref{section proofs hybrid sufficiency} and follows the same ideas as the proof of Theorem \ref{theorem sufficiency}.

\begin{algorithm}[ht]
	\SetAlgoLined
	\SetKwFor{For}{For}{do}{end}
	Each node $v$ has binary input $\mathtt{input}_v \in \set{ 0, 1 }$ and maintains a binary state $\gamma_v \in \set{ 0, 1 }$.\\
	Initially, $\gamma_v := \mathtt{input}_v$.\\
	\For{every \emph{candidate strong faulty} set $T \subseteq V$ such that $\abs{T} \le t$ and every \emph{candidate weak faulty} set $F \subseteq V - T$ such that $\abs{F} \le f$}{
		\begin{enumerate}
			[label=Step (\alph*),topsep=0pt,labelindent=12pt,leftmargin=!]
			\item
			Flood $\gamma_v$ with label $(T, F)$.
			In the remaining steps of the iteration, values\\ received with label $(T, F)$ are considered implicitly.
			
			\item
			For each node $u \in V - T$, identify a single $uv$-path $P_{uv}$ that excludes $T \cup F$.\\
			Set
			\begin{align*}
			Z_v &:= \set{ u \in V - T \mid \text{$v$ received $0$ from $u$ along $P_{uv}$ in step (a)} },\\
			N_v &:= \set{ u \in V - T \mid \text{$v$ received $1$ from $u$ along $P_{uv}$ in step (a)} }.
			\end{align*}
			
			\item
			Define $A_v$ and $B_v$ as follows.
			\begin{enumerate}
				[label=Case \arabic*:,topsep=0pt,labelindent=0pt]
				\item $\abs{Z_v \cap F} \le \floor{f/2}$ and $\abs{N_v} > f + t$.
				Set $A_v := N_v$ and $B_v := Z_v$.
				
				\item $\abs{Z_v \cap F} \le \floor{f/2}$ and $\abs{N_v} \le f + t$.
				Set $A_v := Z_v$ and $B_v := N_v$.
				
				\item $\abs{Z_v \cap F} > \floor{f/2}$ and $\abs{Z_v} > f + t$.
				Set $A_v := Z_v$ and $B_v := N_v$.
				
				\item $\abs{Z_v \cap F} > \floor{f/2}$ and $\abs{Z_v} \le f + t$.
				Set $A_v := N_v$ and $B_v := Z_v$.
			\end{enumerate}
			If $v \in T \cup A_v$, then $\gamma_v$ stays unchanged.
			If $v \in B_v$, then identify $f + t + 1$\\ node-disjoint $A_v v$-paths that exclude $F$.
			If $v$ received identically $0$ (resp. $1$)\\ along these $f + t + 1$ paths in step (a), then set $\gamma_v$ to be $0$ (resp. $1$);\\ otherwise $\gamma_v$ stays unchanged.
		\end{enumerate}
	}
	
	Output $\gamma_v$.
	
	\caption{
		Algorithm for Byzantine Consensus under local broadcast model. All steps are performed by a node $v$.
	}
	\label{algorithm hybrid consensus}
\end{algorithm}
